Explicit, Implicit, and Scattered: Revisiting Event Extraction to Capture Complex Arguments

Prior works formulate the extraction of event-specific arguments as a span extraction problem, where event arguments are explicit -- i.e. assumed to be contiguous spans of text in a document. In this study, we revisit this definition of Event Extraction (EE) by introducing two key argument types that cannot be modeled by existing EE frameworks. First, implicit arguments are event arguments which are not explicitly mentioned in the text, but can be inferred through context. Second, scattered arguments are event arguments that are composed of information scattered throughout the text. These two argument types are crucial to elicit the full breadth of information required for proper event modeling. To support the extraction of explicit, implicit, and scattered arguments, we develop a novel dataset, DiscourseEE, which includes 7,464 argument annotations from online health discourse. Notably, 51.2% of the arguments are implicit, and 17.4% are scattered, making DiscourseEE a unique corpus for complex event extraction. Additionally, we formulate argument extraction as a text generation problem to facilitate the extraction of complex argument types. We provide a comprehensive evaluation of state-of-the-art models and highlight critical open challenges in generative event extraction. Our data and codebase are available at https://omar-sharif03.github.io/DiscourseEE.

==> sections/1.1-Introduction.tex <==
% V2

Event extraction (EE) is best understood as the composition of two core NLP tasks: (i) Event Detection (ED), identifying \textit{if} an event occurs in a text and (ii) Event Argument Extraction (EAE), extracting event-specific details (i.e. event arguments) according to a pre-defined event ontology. 

Existing work in EE has two key limitations. First, most prior works are focused on event modeling of formal texts, such as newspaper or Wikipedia articles. This makes existing EE systems extremely limited in their capacity to model emerging text sources such as social media data, where rich event information is veiled behind informal social discourse. Insufficient data for EE on social media limits the ability of EE to facilitate downstream tasks such as social information extraction, misinformation detection, and characterization of user behaviors. 

Second, existing works in EAE frame argument extraction as a \textit{span extraction} problem --- meaning the event-specific details of interest must be found as substrings of a given document. This is extremely limiting as many key event arguments are implicit and only discernible from subtext. For example, in Figure 1, if one is interested in extracting the ``Goal Dosage" from a social media post, 0mg is only understood as the subtext of the users desire to quit. 

In this paper, we address these two limitations by introducing a novel dataset, DiscourseEE --- which contains EE annotation for health-related discourse on Reddit. By focusing on health discourse, we can provide a nuanced understanding of healthcare needs which has significant implications for public health research \cite{parekh2024event, sharif2023characterizing, guzman-nateras-etal-2022-event}. 

DiscourseEE introduces a novel EE annotation strategy that facilitates the extraction of the following argument types: 

\begin{itemize}
    \item Explicit Arguments: Event details that are found directly in the document. 
    \item Implicit Arguments: Event details which are \textit{not} found in the document but must be inferred using context. 
    \item Scattered Arguments: Event details which are the composition of multiple pieces of information scattered throughout the text. 
\end{itemize}

While there is significant prior work on the extraction of explicit arguments, DiscourseEE is the first task to introduce implicit and scattered argument extraction into EE. When compared to prior work, our EE formulation adds significant depth to the amount of event information which can be extracted, making DiscourseEE well-suited to improve a range of downstream health modeling tasks such as health question-answering, advice modeling (cite conflict paper?), identifying knowledge gaps, and detecting potential misinformation \cite{wu-etal-2022-cross}. Additionally, by changing the EAE paradigm from span extraction to text generation, we better align EE with abilities of Large Language Models which have been shown to have limited capacity on extractive EE tasks (cite). 

Our contributions are as follows: 

1,2,3 



==> sections/misc.tex <==
\section{Task Definition and Event-Schema Design \textcolor{red}{no need to check, working on it!!}}
Our corpus comprises samples from Reddit, an anonymized data source with rich content on MOUD \cite{chancellor}. Following prior work \cite{sharif2023characterizing}, we consider three main event types: \textit{Taking MOUD},  \textit{Relapse or resume MOUD}, and \textit{Tapering}. These events best characterize the advice related to opioid use disorder (OUD) in online health discourse. 

Usually, events consist of a \textit{trigger} and several \textit{arguments} \cite{doddington-etal-2004-automatic, du-cardie-2020-event,lu-etal-2023-event}. The trigger is a word or phrase that best indicates the occurrence of an event and helps to recognize/categorize events, while arguments specify the information characterizing the event. However, detecting event triggers is non-essential to this task \cite{liu-etal-2019-event, tong-etal-2022-docee}. It is time-consuming for annotators to pick out accurate trigger words from a long sentence, which limits the need for trigger identification for this task. Moreover, errors in trigger classification propagate to the subsequent arguments extraction step \cite{liu-etal-2019-event}. 

Without event triggers, it is intuitive to model this task as a multi-label text classification problem. Each sample could have one or multiple target event types.  Nonetheless, arguments are very crucial to characterize the events. We organize the arguments into two hierarchical levels, namely main and sub-arguments, to capture the nuances associated with each event type \cite{sun-etal-2022-phee}. The main arguments are longer text spans that contain details of an event aspect, making it more explainable to humans. Sub-arguments are words or short phrases that highlight specific details of the main arguments. Sub-arguments provide us with the dimensions to compare health advice and find the information overlap or divergence between the advice.      



%Intro version-1

%V-1



\section{Introduction}
Social media sites have become popular platforms for sharing and exchanging information on diverse topics \cite{}. Analyzing this rich information through the lens of event arguments can offer us valuable insights. While most prior work on event extraction has concentrated on news articles or Wikipedia, there has been limited exploration of event extraction from social media data \cite{huang2024textee,tong-etal-2022-docee,du-cardie-2020-event}. One major barrier to this limited exploration is the scarcity of datasets. Event-argument annotation is cognitively demanding and time-consuming, particularly due to the varying spans and vague boundaries of arguments in social media texts \cite{jain-etal-2016-towards}. Additionally, the presence of implicit and scattered arguments further complicates the task, as traditional span-based annotation can not capture them \cite{liu-etal-2021-machine}. This underscores the need for a new annotation approach, benchmark datasets, and models for event extraction from social discourse. To address this need, we developed a novel event ontology, an annotation framework, and a novel discourse-level event extraction dataset \textbf{DiscourseEE}, comprising health discourse from Reddit.

\begin{figure}[t!]
  \centering
  \includegraphics[width =0.95\linewidth]{figures/EAE-example-post.png}
 \caption{An advice-seeking post regarding tapering from opioid use disorder with possible event arguments}
 \label{intro-example-post}
\end{figure}

DiscourseEE consists of health-related information seeking posts and corresponding advice from peers. We focus on health discourse due to its significant societal impact. Analyzing health discourse through the event-argument lens can provide a nuanced understanding of information needs \cite{parekh2024event, sharif2023characterizing, guzman-nateras-etal-2022-event}.
\textcolor{blue}{Need citations for these downstream tasks.} This can benefit various downstream tasks, such as health question-answering \cite{jiang2024covid}, advice modeling \cite{HCD_paper}, and detecting potential misinformation \cite{wu-etal-2022-cross}. From an event-extraction perspective, such discourse consists of complex event arguments and subjective (often ambiguous) forms of arguments with varying spans, implicit and scattered arguments. Therefore, the dataset and models built on this offer a novel resource to explore this avenue in the future.

\textcolor{blue}{advice seeking or information seeking? we should be consistent: Sarah will circle back after the full read.}

\textcolor{blue}{Event argument extraction for social discourse is challenging, as it might need defining event specific ontology, and reliable annotation of the arguments. Figure \ref{intro-example-post} illustrates possible arguments for advice-seeking posts. Here, the individual says that his/her son wants to quit Suboxone, a medication used to treat opioid use disorder (?). }The argument `male' is implicit which is crucial information to provide health advice. Similarly, extracting scattered arguments allows us to get more details about the subject. Explicit arguments can be annotated with a span-based approach, not implicit or scattered ones. Our proposed approach of annotating arguments as natural texts offers flexibility in all three types of downstream argument extraction tasks: \textbf{explicit} (continuous text spans), \textbf{implicit} (not direct mention of arguments), and \textbf{scattered} (a single argument value dispersed throughout the document). Additionally, recent studies suggest incorporating Large Language Models (LLMs) in the annotation process can enhance the quality and speed of annotation \cite{ziems2024large}. Reformulating the annotation as generation aligns with LLM's objective and facilitates the incorporation of LLM in the annotation pipeline. Our major contributions are as follows. 


\begin{itemize}
    \item We introduce event extraction for characterizing discourse-level self-narrarted health advice/information in  social media data/ online discourse. We develop a health-advice-tailored event ontology and a dataset with 7,464 event argument annotations. To the best of our knowledge, this is the largest and most comprehensively annotated discourse-level event extraction dataset with fine-grained annotation. \textcolor{blue}{Should we also mention sub-argument here?} \textcolor{orange}{[ we referred everything as arguments do not mention any sub-arguments term. The reason for this is we annotated all the arguments from post-comment pairs. Our annotation was not hierarchical. For example, if we annotated the subject arguments (age, gender) from the main arguments, then we might call them sub-arguments. Since everything were annotated from post-comment pair I did not use sub-argument term]}
    
    \item We formulate the problem of implicit and scattered argument extraction from online discourse. The problem of implicit and scattered argument has limited exploration previously because of demanding annotation and the model's limited generation capability. %With the advent of generative models understanding of complex contexts improved significantly.  
    % We annotate arguments as natural texts to address the implicit and scattered argument extraction problem. 
    DiscourseEE includes scattered and implicit argument annotations as natural text, providing a novel resource for exploring this avenue in the future.
    \item We benchmark the tasks using a wide range of state-of-the-art event-extraction models on DiscourseEE, including extractive models and advanced large language models (LLMs). We demonstrate the strengths and weaknesses of current models and evaluation challenges of generative event extraction.  
\end{itemize}



%Old tables
\begin{table*}[h!]
\small
\centering
\renewcommand*{\arraystretch}{0.95}

\begin{tabular}{l|ccc|ccc|ccc|c}

 & \multicolumn{3}{c}{\textbf{Taking MOUD}}& \multicolumn{3}{c}{\textbf{Relapse}} & \multicolumn{3}{c}{\textbf{Tapering}}& \\
\midrule
\textbf{Model}& C-A & TS-A & SE-A & C-A & TS-A & SE-A  & C-A & TS-A & SE-A & Mean (RM\_F1)\\
\midrule
Extractive-QA & 4.99 & 19.27 & 16.08 & 14.95 & 29.16 & 15.39 & 19.98 & 18.66 & 15.75 & 17.13\\ 
Generative-QA & &&& &&& &&& \\
-- FLAN-T5 (Base) &  34.99 & 37.23 & 11.41 & 25.38 & 20.31 & 11.38 & 38.78 & 40.94 & 17.54 & 26.44\\
-- FLAN-T5 (Large) & \underline{41.70} & 45.62 & 23.93 & 38.44 & 27.41 & 19.80 & 44.04 & \underline{51.92} & 26.93 & 35.53\\
\midrule
\multicolumn{11}{c}{\textbf{LLMs with Zero-Shot Description-guided Prompt}}\\
\midrule
Gemma (7B) & 28.01 & 36.11 & 31.34 & 20.85 & 30.95 & 33.98 & 28.32 & 27.66 & 27.73 & 29.44\\
 Mixtral (8x7B) & 34.32 & 30.08 & \underline{39.49} & 34.30 & 33.02 & 32.72 & 40.49 & 42.58 & 40.70 & 36.41\\
 Llama-3 (8B) & 33.38 & \underline{47.93} & 34.86 & 33.29 & 37.75 & 27.49 & 42.16 & 42.89 & 35.55 & 37.26\\
Llama-3 (70B) & 37.34 & 38.20 & 27.97 & 38.53 & 33.85 & 25.89 & \underline{45.76} &41.09 & 24.09 & 34.74\\
GPT-4 & 36.00 & 47.54 & 31.32 & \underline{44.81} & \underline{44.23} & 37.01 & 43.93 & 40.60 & 40.65 & 40.68 \\
\midrule
\multicolumn{11}{c}{\textbf{LLMs with Zero-Shot Question-guided Prompt}}\\
\midrule
Gemma (7B) & 22.18 & 46.72 & 24.81 & 15.46 & 34.67 & 22.65 & 29.01 & 37.03 & 28.24 & 28.97\\
Mixtral (8x7B) & 36.36 & 28.14 & 31.53 & 30.84 & 32.89 & 20.67 & 34.47 & 34.15 & 43.45 & 32.50\\
Llama-3 (8B) & 35.38 & 43.09 & 27.35 & 32.79 & 31.59 & 31.54 & 26.42 & 45.89 & 41.09 & 35.01\\
Llama-3 (70B) & 37.24 & 41.47 & 27.46 & 31.50 & 35.50 & 35.37 & 36.95 & 40.16 & 31.86 & 35.28\\
GPT-4 & 35.14 & 47.37 & 37.26 & 43.62 & 40.64 & \underline{49.25} & 39.70 & 45.90 & \underline{44.53} & \textbf{42.60}\\

\bottomrule 
\end{tabular}
\caption{Performance of the models for event argument extraction across all argument types in relaxed match F1-score (RM\_F1). C-A, TS-A, and SE-A denote core, type-specific, and subject-effect arguments. The mean RM\_F1 is calculated by averaging the scores across all argument types for all three classes. The best score in each column is underlined. Model superiority is determined based on the mean RM\_F1 score. Models performance based on exact match F1-score (EM\_F1) presented at table \ref{exact-match-argument-results}.}

\label{relaxed-match-argument-results}
\end{table*}


\begin{table}[t!]
\small
\centering
\renewcommand*{\arraystretch}{0.95}

\begin{tabular}{l|ccc}
& \textbf{P}& \textbf{R} & \textbf{F1} \\
\toprule
\multicolumn{4}{c}{\textbf{Transformer-based Models}}\\
\midrule
BERT & 48.68 & 51.95 & 49.86 \\
MPNet & 46.55 & 63.49 & 52.91\\
RoBERTa & 51.49 & 56.95 & 53.84\\
%XLNet & 27.86 & 41.39 & 33.30\\
\midrule
\multicolumn{4}{c}{\textbf{Instruction-tuned Models}}\\
\midrule
FLAN-T5 (base) & 57.79 & 57.74 & 51.13\\
FLAN-T5 (large) & 56.68 & 54.80 & 55.43 \\
\midrule
\multicolumn{4}{c}{\textbf{LLMs with Zero-Shot Prompt}}\\
\midrule
Gemma-7B & 56.45 & 57.04 & 50.89\\
Mixtral-8x7B & 55.06 & 54.31 & 51.81\\
Llama3-8B & 60.73 & 59.29 & 55.38\\
Llama3-70B & 61.21 & 62.38 & 59.84\\
GPT-4 & 63.50 & 65.72 & \textbf{62.42}\\

\bottomrule
\end{tabular}
\caption{Perfromance comparison of the models for event detection (ED). P, R, and F1 indicate precision, recall, and macro-F1 scores, respectively.}
\label{ed-results}
\end{table}



\begin{table*}[h!]
\small
\centering
\renewcommand*{\arraystretch}{1}

\begin{tabular}{l|ccc|ccc|ccc|c}

 & \multicolumn{3}{c}{\textbf{Taking MOUD}}& \multicolumn{3}{c}{\textbf{Relapse}} & \multicolumn{3}{c}{\textbf{Tapering}}& \\
\midrule
\textbf{Model}& C-A & TS-A & SE-A & C-A & TS-A & SE-A  & C-A & TS-A & SE-A & Mean (EM\_F1)\\
\midrule
Extractive-QA & 1.25 & 7.83 & 1.50 & 3.36 & 14.85 & 6.47 & 5.11 & 4.20 & 4.00 & 5.40\\ 
Generative-QA & &&& &&& &&& \\
-- FLAN-T5 (Base) & 4.89 & 25.24 & 2.85 & 3.75 & 13.31 & 11.37 & 7.40 & 21.93 & 6.67 & 10.82 \\
-- FLAN-T5 (Large) & 5.10 & 32.33 & 7.87 & 7.09 & 18.57 & 14.66 & 10.06 & 33.58 & 10.81 & 15.56\\
\midrule
\multicolumn{11}{c}{\textbf{LLMs with Zero-Shot Description-guided Prompt}}\\
\midrule
Gemma (7B) & 2.35 & 20.88 & 14.21 & 1.11 & 16.33 & 12.65 & 8.45 & 17.76 & 12.57 & 11.81\\
 Mixtral (8x7B) & 7.25 & 18.34 & 11.41 & 3.80 & 13.12 & 12.17 & 8.79 & 19.01 & 11.68 & 11.73 \\
 Llama-3 (8B) & 2.34 & 28.88 & 9.79 & 4.42 & 19.05 & 13.86 & 8.20 & 25.89 & 15.24 & 14.18 \\
Llama-3 (70B) & 6.75 & 25.39 & 9.70 & 5.63 & 21.04 & 13.17 & 11.09 & 22.14 & 15.30 & 14.47 \\
GPT-4 & 2.36 & 27.30 & 14.79 & 7.39 & 23.04 & 21.04 & 8.42 & 20.35 & 16.77 & 15.72 \\
\midrule
\multicolumn{11}{c}{\textbf{LLMs with Zero-Shot Question-guided Prompt}}\\
\midrule
Gemma (7B) & 3.47 & 26.85 & 9.48 & 0.70 & 19.74 & 14.04 & 1.74 & 21.52 & 15.66 & 12.58 \\
Mixtral (8x7B) & 6.17 & 15.94 & 9.59 & 1.56 & 12.74 & 10.86 & 7.71 & 17.39 & 16.46 & 10.93 \\
Llama-3 (8B) & 1.85 & 21.72 & 6.99 & 4.92 & 18.88 & 11.77 & 5.81 & 25.75 & 14.31 & 12.45 \\
Llama-3 (70B) & 3.33 & 25.84 & 10.21 & 5.82 & 23.33 & 14.62 & 12.11 & 23.02 & 18.56 & 15.20 \\
GPT-4 & 4.95 & 29.06 & 19.35 & 6.22 & 21.19 & 26.10 & 8.72 & 21.06 & 14.86 & 16.84 \\
\bottomrule 
\end{tabular}
\caption{Performance of the models for event argument extraction across all argument types in exact match F1-score (EM\_F1).
%M-A, ES-A, and SE-A denote main, event-specific, and subject-effect argument types. The mean RM\_F1 is calculated by averaging the scores across all argument types for all three classes. Model superiority is determined based on the mean RM\_F1 score.\textcolor{red}{We have more experimental results. (Such as isolated question-guided and description-guided). Due to space I am not planning to add it in the main paper. Can discuss more. }
}

\label{exact-match-argument-results}
\end{table*}



\begin{table}[h]
\small
\centering
\renewcommand*{\arraystretch}{1}

\begin{tabular}{l|ccc}

 & \multicolumn{3}{c}{\textbf{Relaxed Match (Recall)}}\\
\midrule
\textbf{Model}& Explicit & Implicit & Scattered \\
\midrule
Extractive-QA & 32.40 & 9.40 & 13.44  \\ 
Generative-QA &&& \\
-- FLAN-T5 (Base) & 35.49 & 23.72 & 33.33 \\
-- FLAN-T5 (Large) & 45.98& 34.15& 43.54 \\
\midrule
\multicolumn{4}{c}{\textbf{LLMs with Zero-Shot Description-guided Prompt}}\\
\midrule
Gemma (7B) & 37.34 & 23.31 & 29.03 \\
 Mixtral (8x7B) & 52.77 & 28.01 & 48.38 \\
 Llama-3 (8B)  & 46.29 & 31.69 & 39.24 \\
Llama-3 (70B)  & 50.00 & 26.99 & 41.93  \\
GPT-4  & 53.39 & 33.12 & \textbf{55.37} \\
\midrule
\multicolumn{4}{c}{\textbf{LLMs with Zero-Shot Question-guided Prompt}}\\
\midrule
Gemma (7B)  & 41.66 & 23.10 & 26.34 \\
 Mixtral (8x7B)  & 48.54 & 26.58 & 49.46 \\
 Llama-3 (8B) & 41.35 & 30.67 & 37.09 \\
Llama-3 (70B)  & 50.00 & 29.03 &36.02  \\
GPT-4  & \textbf{57.09} & \textbf{36.60} & 50.53 \\
\bottomrule 
\end{tabular}
\caption{Performance comparison of explicit, implicit, and scattered argument extraction. Model performance (avg. of 3 runs) is reported based on recall, showing how many explicit, implicit, and scattered arguments are extracted correctly.
}



\begin{table}[h!]
\small
\centering
\renewcommand*{\arraystretch}{1}

\begin{tabular}{l|ccc}

 & \multicolumn{3}{c}{\textbf{Exact Match (Recall)}}\\
\midrule
\textbf{Model}& Explicit & Implicit & Scattered \\
\midrule
Extractive-QA & 20.67 & 0.40 & 0.0  \\ 
Generative-QA &&& \\
-- FLAN-T5 (Base) & 26.54 & 10.02 & 1.61 \\
-- FLAN-T5 (Large) & 33.33 & 14.72 & 5.91 \\
\midrule
\multicolumn{4}{c}{\textbf{LLMs with Zero-Shot Description-guided Prompt}}\\
\midrule
Gemma (7B) & 27.77 & 7.56 & 0.53 \\
 Mixtral (8x7B) & 34.56 & 6.54 & 3.22 \\
 Llama-3 (8B)  & 33.64 & 10.22 & 1.07 \\
Llama-3 (70B)  &  37.03 & 7.36 & 3.23 \\
GPT-4  &  37.96 & 10.63 & 3.22\\
\midrule
\multicolumn{4}{c}{\textbf{LLMs with Zero-Shot Question-guided Prompt}}\\
\midrule
Gemma (7B)  & 32.09 & 6.95 & 1.61 \\
 Mixtral (8x7B)  &  31.17 & 7.56 & 2.68\\
 Llama-3 (8B) &  30.86 & 8.58 & 1.61\\
Llama-3 (70B)  & 40.12 & 8.99 & 1.61  \\
GPT-4  &  39.50 & 12.06 & 3.22\\
\bottomrule 
\end{tabular}
\caption{Performance comparison of explicit, implicit, and scattered argument extraction in exact-match setting. Performance drop is significant in scattered arguments as these arguments are longer. Models generate different outputs with slight variation, which is not considered under exact match. 
}

%Model performance is reported based on a percentage of explicit, implicit, and scattered arguments predicted accurately. 
\label{exact-match-explicit-implicit-scattered-argument-results}
\end{table}

